Transfer-LMR: Heavy-Tail Driving Behavior Recognition in Diverse Traffic Scenarios

Recognizing driving behaviors is important for downstream tasks such as reasoning, planning, and navigation. Existing video recognition approaches work well for common behaviors (e.g. "drive straight", "brake", "turn left/right"). However, the performance is sub-par for underrepresented/rare behaviors typically found in tail of the behavior class distribution. To address this shortcoming, we propose Transfer-LMR, a modular training routine for improving the recognition performance across all driving behavior classes. We extensively evaluate our approach on METEOR and HDD datasets that contain rich yet heavy-tailed distribution of driving behaviors and span diverse traffic scenarios. The experimental results demonstrate the efficacy of our approach, especially for recognizing underrepresented/rare driving behaviors.

==> figs/meteor_data_samples.tex <==

\begin{figure*}[t]
\centering
   \begin{subfigure}[h]{\textwidth}
    \includegraphics[width=\textwidth]{figs/METEOR_samples1.pdf}
    \vspace*{-0.2in}
    \caption{\textbf{Cutting:} Ego vehicle crosses the three-wheeler's path on the right side of the road.}
    \label{fig: sample1}
    \vspace{5pt}
  \end{subfigure}
  %
 \begin{subfigure}[h]{\textwidth}
    \includegraphics[width=\textwidth]{figs/METEOR_samples2.pdf}
    \vspace*{-0.2in}
    \caption{\textbf{Yielding:} Ego vehicle slows down due to obstruction in its path by the crossing motorcycle.}
    \label{fig: sample2}
    \vspace{5pt}
  \end{subfigure}
 %
   \begin{subfigure}[h]{\textwidth}
    \includegraphics[width=\textwidth, height=2.32cm]{figs/METEOR_samples3.pdf}
    \vspace*{-0.2in}
    \caption{\textbf{Wrong Lane:} Ego vehicle tries to move ahead of the truck by deviating from its path towards the oncoming vehicles' lane. }
    \label{fig: sample3}
    \vspace{5pt}
  \end{subfigure}
  %
  \begin{subfigure}[h]{\textwidth}
 % \begin{subfigure}[h]{0.245\textwidth}
    \includegraphics[width=\textwidth]{figs/METEOR_samples4.pdf}
    \vspace*{-0.2in}
    \caption{\textbf{Overtaking:} Ego vehicle moves ahead of the bus while staying in the correct lane. }
    \label{fig: sample4}
    \vspace{5pt}
  \end{subfigure}
 
\caption{\textbf{METEOR dataset:} Atypical Ego Vehicle's Driving Behaviors sample driving scenarios. The keyframes of the driving scenarios are shown along with its bird's eye view illustration on the right side. The red-colored rectangle is the ego vehicle and the blue-colored rectangles are road agents. The left lane is the ego's driving lane while the right lane is the oncoming vehicles' lane.}
  \label{fig: dataset_diagram}
  \vspace{-10pt}
\end{figure*}


